Search for charged Higgs bosons in top quark decays

We present a search for charged Higgs bosons in top quark decays. We analyze the \eplus, \muplus, $ee$, $e\mu$, $\mu\mu$, \etau and \mutau final states from top quark pair production events, using data from about 1${\text{fb}}^{-1}$ of integrated luminosity recorded by the \dzero experiment at the Fermilab Tevatron Collider. We consider different scenarios of possible charged Higgs boson decays, one where the charged Higgs boson decays purely hadronically into a charm and a strange quark, another where it decays into a $\tau$ lepton and a $\tau$ neutrino and a third one where both decays appear. We extract limits on the branching ratio $B(t\to H^+ b)$ for all these models. We use two methods, one where the $t\bar{t}$ production cross section is fixed, and one where the cross section is fitted simultaneously with $B(t\to H^+b)$. Based on the extracted limits, we exclude regions in the charged Higgs boson mass and $\tan \beta$ parameter space for different scenarios of the minimal supersymmetric standard model.

==> acknowledgement_paragraph_r2.tex <==
% acknowledgement_paragraph_r2.tex                         7/7/09
%
We thank the staffs at Fermilab and collaborating institutions, 
and acknowledge support from the 
DOE and NSF (USA);
CEA and CNRS/IN2P3 (France);
FASI, Rosatom and RFBR (Russia);
CNPq, FAPERJ, FAPESP and FUNDUNESP (Brazil);
DAE and DST (India);
Colciencias (Colombia);
CONACyT (Mexico);
KRF and KOSEF (Korea);
CONICET and UBACyT (Argentina);
FOM (The Netherlands);
STFC and the Royal Society (United Kingdom);
MSMT and GACR (Czech Republic);
CRC Program, CFI, NSERC and WestGrid Project (Canada);
BMBF and DFG (Germany);
SFI (Ireland);
The Swedish Research Council (Sweden);
CAS and CNSF (China);
and the
Alexander von Humboldt Foundation (Germany).
%


==> list_of_authors_r2.tex <==
% LIST_OF_AUTHORS_R2.TEX                 7/7/09             
%
\author{V.M.~Abazov$^{37}$}
\author{B.~Abbott$^{75}$}
\author{M.~Abolins$^{65}$}
\author{B.S.~Acharya$^{30}$}
\author{M.~Adams$^{51}$}
\author{T.~Adams$^{49}$}
\author{E.~Aguilo$^{6}$}
\author{M.~Ahsan$^{59}$}
\author{G.D.~Alexeev$^{37}$}
\author{G.~Alkhazov$^{41}$}
\author{A.~Alton$^{64,a}$}
\author{G.~Alverson$^{63}$}
\author{G.A.~Alves$^{2}$}
\author{L.S.~Ancu$^{36}$}
\author{M.S.~Anzelc$^{53}$}
\author{M.~Aoki$^{50}$}
\author{Y.~Arnoud$^{14}$}
\author{M.~Arov$^{60}$}
\author{M.~Arthaud$^{18}$}
\author{A.~Askew$^{49,b}$}
\author{B.~{\AA}sman$^{42}$}
\author{O.~Atramentov$^{49,b}$}
\author{C.~Avila$^{8}$}
\author{J.~BackusMayes$^{82}$}
\author{F.~Badaud$^{13}$}
\author{L.~Bagby$^{50}$}
\author{B.~Baldin$^{50}$}
\author{D.V.~Bandurin$^{59}$}
\author{S.~Banerjee$^{30}$}
\author{E.~Barberis$^{63}$}
\author{A.-F.~Barfuss$^{15}$}
\author{P.~Bargassa$^{80}$}
\author{P.~Baringer$^{58}$}
\author{J.~Barreto$^{2}$}
\author{J.F.~Bartlett$^{50}$}
\author{U.~Bassler$^{18}$}
\author{D.~Bauer$^{44}$}
\author{S.~Beale$^{6}$}
\author{A.~Bean$^{58}$}
\author{M.~Begalli$^{3}$}
\author{M.~Begel$^{73}$}
\author{C.~Belanger-Champagne$^{42}$}
\author{L.~Bellantoni$^{50}$}
\author{A.~Bellavance$^{50}$}
\author{J.A.~Benitez$^{65}$}
\author{S.B.~Beri$^{28}$}
\author{G.~Bernardi$^{17}$}
\author{R.~Bernhard$^{23}$}
\author{I.~Bertram$^{43}$}
\author{M.~Besan\c{c}on$^{18}$}
\author{R.~Beuselinck$^{44}$}
\author{V.A.~Bezzubov$^{40}$}
\author{P.C.~Bhat$^{50}$}
\author{V.~Bhatnagar$^{28}$}
\author{G.~Blazey$^{52}$}
\author{S.~Blessing$^{49}$}
\author{K.~Bloom$^{67}$}
\author{A.~Boehnlein$^{50}$}
\author{D.~Boline$^{62}$}
\author{T.A.~Bolton$^{59}$}
\author{E.E.~Boos$^{39}$}
\author{G.~Borissov$^{43}$}
\author{T.~Bose$^{62}$}
\author{A.~Brandt$^{78}$}
\author{R.~Brock$^{65}$}
\author{G.~Brooijmans$^{70}$}
\author{A.~Bross$^{50}$}
\author{D.~Brown$^{19}$}
\author{X.B.~Bu$^{7}$}
\author{D.~Buchholz$^{53}$}
\author{M.~Buehler$^{81}$}
\author{V.~Buescher$^{22}$}
\author{V.~Bunichev$^{39}$}
\author{S.~Burdin$^{43,c}$}
\author{T.H.~Burnett$^{82}$}
\author{C.P.~Buszello$^{44}$}
\author{P.~Calfayan$^{26}$}
\author{B.~Calpas$^{15}$}
\author{S.~Calvet$^{16}$}
\author{J.~Cammin$^{71}$}
\author{M.A.~Carrasco-Lizarraga$^{34}$}
\author{E.~Carrera$^{49}$}
\author{W.~Carvalho$^{3}$}
\author{B.C.K.~Casey$^{50}$}
\author{H.~Castilla-Valdez$^{34}$}
\author{S.~Chakrabarti$^{72}$}
\author{D.~Chakraborty$^{52}$}
\author{K.M.~Chan$^{55}$}
\author{A.~Chandra$^{48}$}
\author{E.~Cheu$^{46}$}
\author{D.K.~Cho$^{62}$}
\author{S.W.~Cho$^{32}$}
\author{S.~Choi$^{33}$}
\author{B.~Choudhary$^{29}$}
\author{T.~Christoudias$^{44}$}
\author{S.~Cihangir$^{50}$}
\author{D.~Claes$^{67}$}
\author{J.~Clutter$^{58}$}
\author{M.~Cooke$^{50}$}
\author{W.E.~Cooper$^{50}$}
\author{M.~Corcoran$^{80}$}
\author{F.~Couderc$^{18}$}
\author{M.-C.~Cousinou$^{15}$}
\author{D.~Cutts$^{77}$}
\author{M.~{\'C}wiok$^{31}$}
\author{A.~Das$^{46}$}
\author{G.~Davies$^{44}$}
\author{K.~De$^{78}$}
\author{S.J.~de~Jong$^{36}$}
\author{E.~De~La~Cruz-Burelo$^{34}$}
\author{K.~DeVaughan$^{67}$}
\author{F.~D\'eliot$^{18}$}
\author{M.~Demarteau$^{50}$}
\author{R.~Demina$^{71}$}
\author{D.~Denisov$^{50}$}
\author{S.P.~Denisov$^{40}$}
\author{S.~Desai$^{50}$}
\author{H.T.~Diehl$^{50}$}
\author{M.~Diesburg$^{50}$}
\author{A.~Dominguez$^{67}$}
\author{T.~Dorland$^{82}$}
\author{A.~Dubey$^{29}$}
\author{L.V.~Dudko$^{39}$}
\author{L.~Duflot$^{16}$}
\author{D.~Duggan$^{49}$}
\author{A.~Duperrin$^{15}$}
\author{S.~Dutt$^{28}$}
\author{A.~Dyshkant$^{52}$}
\author{M.~Eads$^{67}$}
\author{D.~Edmunds$^{65}$}
\author{J.~Ellison$^{48}$}
\author{V.D.~Elvira$^{50}$}
\author{Y.~Enari$^{77}$}
\author{S.~Eno$^{61}$}
\author{M.~Escalier$^{15}$}
\author{H.~Evans$^{54}$}
\author{A.~Evdokimov$^{73}$}
\author{V.N.~Evdokimov$^{40}$}
\author{G.~Facini$^{63}$}
\author{A.V.~Ferapontov$^{59}$}
\author{T.~Ferbel$^{61,71}$}
\author{F.~Fiedler$^{25}$}
\author{F.~Filthaut$^{36}$}
\author{W.~Fisher$^{50}$}
\author{H.E.~Fisk$^{50}$}
\author{M.~Fortner$^{52}$}
\author{H.~Fox$^{43}$}
\author{S.~Fu$^{50}$}
\author{S.~Fuess$^{50}$}
\author{T.~Gadfort$^{70}$}
\author{C.F.~Galea$^{36}$}
\author{A.~Garcia-Bellido$^{71}$}
\author{V.~Gavrilov$^{38}$}
\author{P.~Gay$^{13}$}
\author{W.~Geist$^{19}$}
\author{W.~Geng$^{15,65}$}
\author{C.E.~Gerber$^{51}$}
\author{Y.~Gershtein$^{49,b}$}
\author{D.~Gillberg$^{6}$}
\author{G.~Ginther$^{50,71}$}
\author{B.~G\'{o}mez$^{8}$}
\author{A.~Goussiou$^{82}$}
\author{P.D.~Grannis$^{72}$}
\author{S.~Greder$^{19}$}
\author{H.~Greenlee$^{50}$}
\author{Z.D.~Greenwood$^{60}$}
\author{E.M.~Gregores$^{4}$}
\author{G.~Grenier$^{20}$}
\author{Ph.~Gris$^{13}$}
\author{J.-F.~Grivaz$^{16}$}
\author{A.~Grohsjean$^{18}$}
\author{S.~Gr\"unendahl$^{50}$}
\author{M.W.~Gr{\"u}newald$^{31}$}
\author{F.~Guo$^{72}$}
\author{J.~Guo$^{72}$}
\author{G.~Gutierrez$^{50}$}
\author{P.~Gutierrez$^{75}$}
\author{A.~Haas$^{70}$}
\author{P.~Haefner$^{26}$}
\author{S.~Hagopian$^{49}$}
\author{J.~Haley$^{68}$}
\author{I.~Hall$^{65}$}
\author{R.E.~Hall$^{47}$}
\author{L.~Han$^{7}$}
\author{K.~Harder$^{45}$}
\author{A.~Harel$^{71}$}
\author{J.M.~Hauptman$^{57}$}
\author{J.~Hays$^{44}$}
\author{T.~Hebbeker$^{21}$}
\author{D.~Hedin$^{52}$}
\author{J.G.~Hegeman$^{35}$}
\author{A.P.~Heinson$^{48}$}
\author{U.~Heintz$^{62}$}
\author{C.~Hensel$^{24}$}
\author{I.~Heredia-De~La~Cruz$^{34}$}
\author{K.~Herner$^{64}$}
\author{G.~Hesketh$^{63}$}
\author{M.D.~Hildreth$^{55}$}
\author{R.~Hirosky$^{81}$}
\author{T.~Hoang$^{49}$}
\author{J.D.~Hobbs$^{72}$}
\author{B.~Hoeneisen$^{12}$}
\author{M.~Hohlfeld$^{22}$}
\author{S.~Hossain$^{75}$}
\author{P.~Houben$^{35}$}
\author{Y.~Hu$^{72}$}
\author{Z.~Hubacek$^{10}$}
\author{N.~Huske$^{17}$}
\author{V.~Hynek$^{10}$}
\author{I.~Iashvili$^{69}$}
\author{R.~Illingworth$^{50}$}
\author{A.S.~Ito$^{50}$}
\author{S.~Jabeen$^{62}$}
\author{M.~Jaffr\'e$^{16}$}
\author{S.~Jain$^{75}$}
\author{K.~Jakobs$^{23}$}
\author{D.~Jamin$^{15}$}
\author{R.~Jesik$^{44}$}
\author{K.~Johns$^{46}$}
\author{C.~Johnson$^{70}$}
\author{M.~Johnson$^{50}$}
\author{D.~Johnston$^{67}$}
\author{A.~Jonckheere$^{50}$}
\author{P.~Jonsson$^{44}$}
\author{A.~Juste$^{50}$}
\author{E.~Kajfasz$^{15}$}
\author{D.~Karmanov$^{39}$}
\author{P.A.~Kasper$^{50}$}
\author{I.~Katsanos$^{67}$}
\author{V.~Kaushik$^{78}$}
\author{R.~Kehoe$^{79}$}
\author{S.~Kermiche$^{15}$}
\author{N.~Khalatyan$^{50}$}
\author{A.~Khanov$^{76}$}
\author{A.~Kharchilava$^{69}$}
\author{Y.N.~Kharzheev$^{37}$}
\author{D.~Khatidze$^{77}$}
\author{M.H.~Kirby$^{53}$}
\author{M.~Kirsch$^{21}$}
\author{B.~Klima$^{50}$}
\author{J.M.~Kohli$^{28}$}
\author{J.-P.~Konrath$^{23}$}
\author{A.V.~Kozelov$^{40}$}
\author{J.~Kraus$^{65}$}
\author{T.~Kuhl$^{25}$}
\author{A.~Kumar$^{69}$}
\author{A.~Kupco$^{11}$}
\author{T.~Kur\v{c}a$^{20}$}
\author{V.A.~Kuzmin$^{39}$}
\author{J.~Kvita$^{9}$}
\author{F.~Lacroix$^{13}$}
\author{D.~Lam$^{55}$}
\author{S.~Lammers$^{54}$}
\author{G.~Landsberg$^{77}$}
\author{P.~Lebrun$^{20}$}
\author{H.S.~Lee$^{32}$}
\author{W.M.~Lee$^{50}$}
\author{A.~Leflat$^{39}$}
\author{J.~Lellouch$^{17}$}
\author{L.~Li$^{48}$}
\author{Q.Z.~Li$^{50}$}
\author{S.M.~Lietti$^{5}$}
\author{J.K.~Lim$^{32}$}
\author{D.~Lincoln$^{50}$}
\author{J.~Linnemann$^{65}$}
\author{V.V.~Lipaev$^{40}$}
\author{R.~Lipton$^{50}$}
\author{Y.~Liu$^{7}$}
\author{Z.~Liu$^{6}$}
\author{A.~Lobodenko$^{41}$}
\author{M.~Lokajicek$^{11}$}
\author{P.~Love$^{43}$}
\author{H.J.~Lubatti$^{82}$}
\author{R.~Luna-Garcia$^{34,d}$}
\author{A.L.~Lyon$^{50}$}
\author{A.K.A.~Maciel$^{2}$}
\author{D.~Mackin$^{80}$}
\author{P.~M\"attig$^{27}$}
\author{R.~Maga\~na-Villalba$^{34}$}
\author{P.K.~Mal$^{46}$}
\author{S.~Malik$^{67}$}
\author{V.L.~Malyshev$^{37}$}
\author{Y.~Maravin$^{59}$}
\author{B.~Martin$^{14}$}
\author{R.~McCarthy$^{72}$}
\author{C.L.~McGivern$^{58}$}
\author{M.M.~Meijer$^{36}$}
\author{A.~Melnitchouk$^{66}$}
\author{L.~Mendoza$^{8}$}
\author{D.~Menezes$^{52}$}
\author{P.G.~Mercadante$^{5}$}
\author{M.~Merkin$^{39}$}
\author{K.W.~Merritt$^{50}$}
\author{A.~Meyer$^{21}$}
\author{J.~Meyer$^{24}$}
\author{N.K.~Mondal$^{30}$}
\author{R.W.~Moore$^{6}$}
\author{T.~Moulik$^{58}$}
\author{G.S.~Muanza$^{15}$}
\author{M.~Mulhearn$^{70}$}
\author{O.~Mundal$^{22}$}
\author{L.~Mundim$^{3}$}
\author{E.~Nagy$^{15}$}
\author{M.~Naimuddin$^{50}$}
\author{M.~Narain$^{77}$}
\author{H.A.~Neal$^{64}$}
\author{J.P.~Negret$^{8}$}
\author{P.~Neustroev$^{41}$}
\author{H.~Nilsen$^{23}$}
\author{H.~Nogima$^{3}$}
\author{S.F.~Novaes$^{5}$}
\author{T.~Nunnemann$^{26}$}
\author{G.~Obrant$^{41}$}
\author{C.~Ochando$^{16}$}
\author{D.~Onoprienko$^{59}$}
\author{J.~Orduna$^{34}$}
\author{N.~Oshima$^{50}$}
\author{N.~Osman$^{44}$}
\author{J.~Osta$^{55}$}
\author{R.~Otec$^{10}$}
\author{G.J.~Otero~y~Garz{\'o}n$^{1}$}
\author{M.~Owen$^{45}$}
\author{M.~Padilla$^{48}$}
\author{P.~Padley$^{80}$}
\author{M.~Pangilinan$^{77}$}
\author{N.~Parashar$^{56}$}
\author{S.-J.~Park$^{24}$}
\author{S.K.~Park$^{32}$}
\author{J.~Parsons$^{70}$}
\author{R.~Partridge$^{77}$}
\author{N.~Parua$^{54}$}
\author{A.~Patwa$^{73}$}
\author{B.~Penning$^{23}$}
\author{M.~Perfilov$^{39}$}
\author{K.~Peters$^{45}$}
\author{Y.~Peters$^{45}$}
\author{P.~P\'etroff$^{16}$}
\author{R.~Piegaia$^{1}$}
\author{J.~Piper$^{65}$}
\author{M.-A.~Pleier$^{22}$}
\author{P.L.M.~Podesta-Lerma$^{34,e}$}
\author{V.M.~Podstavkov$^{50}$}
\author{Y.~Pogorelov$^{55}$}
\author{M.-E.~Pol$^{2}$}
\author{P.~Polozov$^{38}$}
\author{A.V.~Popov$^{40}$}
\author{M.~Prewitt$^{80}$}
\author{S.~Protopopescu$^{73}$}
\author{J.~Qian$^{64}$}
\author{A.~Quadt$^{24}$}
\author{B.~Quinn$^{66}$}
\author{A.~Rakitine$^{43}$}
\author{M.S.~Rangel$^{16}$}
\author{K.~Ranjan$^{29}$}
\author{P.N.~Ratoff$^{43}$}
\author{P.~Renkel$^{79}$}
\author{P.~Rich$^{45}$}
\author{M.~Rijssenbeek$^{72}$}
\author{I.~Ripp-Baudot$^{19}$}
\author{F.~Rizatdinova$^{76}$}
\author{S.~Robinson$^{44}$}
\author{M.~Rominsky$^{75}$}
\author{C.~Royon$^{18}$}
\author{P.~Rubinov$^{50}$}
\author{R.~Ruchti$^{55}$}
\author{G.~Safronov$^{38}$}
\author{G.~Sajot$^{14}$}
\author{A.~S\'anchez-Hern\'andez$^{34}$}
\author{M.P.~Sanders$^{26}$}
\author{B.~Sanghi$^{50}$}
\author{G.~Savage$^{50}$}
\author{L.~Sawyer$^{60}$}
\author{T.~Scanlon$^{44}$}
\author{D.~Schaile$^{26}$}
\author{R.D.~Schamberger$^{72}$}
\author{Y.~Scheglov$^{41}$}
\author{H.~Schellman$^{53}$}
\author{T.~Schliephake$^{27}$}
\author{S.~Schlobohm$^{82}$}
\author{C.~Schwanenberger$^{45}$}
\author{R.~Schwienhorst$^{65}$}
\author{J.~Sekaric$^{49}$}
\author{H.~Severini$^{75}$}
\author{E.~Shabalina$^{24}$}
\author{M.~Shamim$^{59}$}
\author{V.~Shary$^{18}$}
\author{A.A.~Shchukin$^{40}$}
\author{R.K.~Shivpuri$^{29}$}
\author{V.~Siccardi$^{19}$}
\author{V.~Simak$^{10}$}
\author{V.~Sirotenko$^{50}$}
\author{P.~Skubic$^{75}$}
\author{P.~Slattery$^{71}$}
\author{D.~Smirnov$^{55}$}
\author{G.R.~Snow$^{67}$}
\author{J.~Snow$^{74}$}
\author{S.~Snyder$^{73}$}
\author{S.~S{\"o}ldner-Rembold$^{45}$}
\author{L.~Sonnenschein$^{21}$}
\author{A.~Sopczak$^{43}$}
\author{M.~Sosebee$^{78}$}
\author{K.~Soustruznik$^{9}$}
\author{B.~Spurlock$^{78}$}
\author{J.~Stark$^{14}$}
\author{V.~Stolin$^{38}$}
\author{D.A.~Stoyanova$^{40}$}
\author{J.~Strandberg$^{64}$}
\author{M.A.~Strang$^{69}$}
\author{E.~Strauss$^{72}$}
\author{M.~Strauss$^{75}$}
\author{R.~Str{\"o}hmer$^{26}$}
\author{D.~Strom$^{51}$}
\author{L.~Stutte$^{50}$}
\author{S.~Sumowidagdo$^{49}$}
\author{P.~Svoisky$^{36}$}
\author{M.~Takahashi$^{45}$}
\author{A.~Tanasijczuk$^{1}$}
\author{W.~Taylor$^{6}$}
\author{B.~Tiller$^{26}$}
\author{M.~Titov$^{18}$}
\author{V.V.~Tokmenin$^{37}$}
\author{I.~Torchiani$^{23}$}
\author{D.~Tsybychev$^{72}$}
\author{B.~Tuchming$^{18}$}
\author{C.~Tully$^{68}$}
\author{P.M.~Tuts$^{70}$}
\author{R.~Unalan$^{65}$}
\author{L.~Uvarov$^{41}$}
\author{S.~Uvarov$^{41}$}
\author{S.~Uzunyan$^{52}$}
\author{P.J.~van~den~Berg$^{35}$}
\author{R.~Van~Kooten$^{54}$}
\author{W.M.~van~Leeuwen$^{35}$}
\author{N.~Varelas$^{51}$}
\author{E.W.~Varnes$^{46}$}
\author{I.A.~Vasilyev$^{40}$}
\author{P.~Verdier$^{20}$}
\author{L.S.~Vertogradov$^{37}$}
\author{M.~Verzocchi$^{50}$}
\author{M.~Vesterinen$^{45}$}
\author{D.~Vilanova$^{18}$}
\author{P.~Vint$^{44}$}
\author{P.~Vokac$^{10}$}
\author{R.~Wagner$^{68}$}
\author{H.D.~Wahl$^{49}$}
\author{M.H.L.S.~Wang$^{71}$}
\author{J.~Warchol$^{55}$}
\author{G.~Watts$^{82}$}
\author{M.~Wayne$^{55}$}
\author{G.~Weber$^{25}$}
\author{M.~Weber$^{50,f}$}
\author{L.~Welty-Rieger$^{54}$}
\author{A.~Wenger$^{23,g}$}
\author{M.~Wetstein$^{61}$}
\author{A.~White$^{78}$}
\author{D.~Wicke$^{25}$}
\author{M.R.J.~Williams$^{43}$}
\author{G.W.~Wilson$^{58}$}
\author{S.J.~Wimpenny$^{48}$}
\author{M.~Wobisch$^{60}$}
\author{D.R.~Wood$^{63}$}
\author{T.R.~Wyatt$^{45}$}
\author{Y.~Xie$^{77}$}
\author{C.~Xu$^{64}$}
\author{S.~Yacoob$^{53}$}
\author{R.~Yamada$^{50}$}
\author{W.-C.~Yang$^{45}$}
\author{T.~Yasuda$^{50}$}
\author{Y.A.~Yatsunenko$^{37}$}
\author{Z.~Ye$^{50}$}
\author{H.~Yin$^{7}$}
\author{K.~Yip$^{73}$}
\author{H.D.~Yoo$^{77}$}
\author{S.W.~Youn$^{50}$}
\author{J.~Yu$^{78}$}
\author{C.~Zeitnitz$^{27}$}
\author{S.~Zelitch$^{81}$}
\author{T.~Zhao$^{82}$}
\author{B.~Zhou$^{64}$}
\author{J.~Zhu$^{72}$}
\author{M.~Zielinski$^{71}$}
\author{D.~Zieminska$^{54}$}
\author{L.~Zivkovic$^{70}$}
\author{V.~Zutshi$^{52}$}
\author{E.G.~Zverev$^{39}$}

\affiliation{\vspace{0.1 in}(The D\O\ Collaboration)\vspace{0.1 in}}
\affiliation{$^{1}$Universidad de Buenos Aires, Buenos Aires, Argentina}
\affiliation{$^{2}$LAFEX, Centro Brasileiro de Pesquisas F{\'\i}sicas,
                Rio de Janeiro, Brazil}
\affiliation{$^{3}$Universidade do Estado do Rio de Janeiro,
                Rio de Janeiro, Brazil}
\affiliation{$^{4}$Universidade Federal do ABC,
                Santo Andr\'e, Brazil}
\affiliation{$^{5}$Instituto de F\'{\i}sica Te\'orica, Universidade Estadual
                Paulista, S\~ao Paulo, Brazil}
\affiliation{$^{6}$University of Alberta, Edmonton, Alberta, Canada;
                Simon Fraser University, Burnaby, British Columbia, Canada;
                York University, Toronto, Ontario, Canada and
                McGill University, Montreal, Quebec, Canada}
\affiliation{$^{7}$University of Science and Technology of China,
                Hefei, People's Republic of China}
\affiliation{$^{8}$Universidad de los Andes, Bogot\'{a}, Colombia}
\affiliation{$^{9}$Center for Particle Physics, Charles University,
                Faculty of Mathematics and Physics, Prague, Czech Republic}
\affiliation{$^{10}$Czech Technical University in Prague,
                Prague, Czech Republic}
\affiliation{$^{11}$Center for Particle Physics, Institute of Physics,
                Academy of Sciences of the Czech Republic,
                Prague, Czech Republic}
\affiliation{$^{12}$Universidad San Francisco de Quito, Quito, Ecuador}
\affiliation{$^{13}$LPC, Universit\'e Blaise Pascal, CNRS/IN2P3,
                Clermont, France}
\affiliation{$^{14}$LPSC, Universit\'e Joseph Fourier Grenoble 1,
                CNRS/IN2P3, Institut National Polytechnique de Grenoble,
                Grenoble, France}
\affiliation{$^{15}$CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3,
                Marseille, France}
\affiliation{$^{16}$LAL, Universit\'e Paris-Sud, IN2P3/CNRS, Orsay, France}
\affiliation{$^{17}$LPNHE, IN2P3/CNRS, Universit\'es Paris VI and VII,
                Paris, France}
\affiliation{$^{18}$CEA, Irfu, SPP, Saclay, France}
\affiliation{$^{19}$IPHC, Universit\'e de Strasbourg, CNRS/IN2P3,
                Strasbourg, France}
\affiliation{$^{20}$IPNL, Universit\'e Lyon 1, CNRS/IN2P3,
                Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\affiliation{$^{21}$III. Physikalisches Institut A, RWTH Aachen University,
                Aachen, Germany}
\affiliation{$^{22}$Physikalisches Institut, Universit{\"a}t Bonn,
                Bonn, Germany}
\affiliation{$^{23}$Physikalisches Institut, Universit{\"a}t Freiburg,
                Freiburg, Germany}
\affiliation{$^{24}$II. Physikalisches Institut, Georg-August-Universit{\"a}t
                G\"ottingen, G\"ottingen, Germany}
\affiliation{$^{25}$Institut f{\"u}r Physik, Universit{\"a}t Mainz,
                Mainz, Germany}
\affiliation{$^{26}$Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen,
                M{\"u}nchen, Germany}
\affiliation{$^{27}$Fachbereich Physik, University of Wuppertal,
                Wuppertal, Germany}
\affiliation{$^{28}$Panjab University, Chandigarh, India}
\affiliation{$^{29}$Delhi University, Delhi, India}
\affiliation{$^{30}$Tata Institute of Fundamental Research, Mumbai, India}
\affiliation{$^{31}$University College Dublin, Dublin, Ireland}
\affiliation{$^{32}$Korea Detector Laboratory, Korea University, Seoul, Korea}
\affiliation{$^{33}$SungKyunKwan University, Suwon, Korea}
\affiliation{$^{34}$CINVESTAV, Mexico City, Mexico}
\affiliation{$^{35}$FOM-Institute NIKHEF and University of Amsterdam/NIKHEF,
                Amsterdam, The Netherlands}
\affiliation{$^{36}$Radboud University Nijmegen/NIKHEF,
                Nijmegen, The Netherlands}
\affiliation{$^{37}$Joint Institute for Nuclear Research, Dubna, Russia}
\affiliation{$^{38}$Institute for Theoretical and Experimental Physics,
                Moscow, Russia}
\affiliation{$^{39}$Moscow State University, Moscow, Russia}
\affiliation{$^{40}$Institute for High Energy Physics, Protvino, Russia}
\affiliation{$^{41}$Petersburg Nuclear Physics Institute,
                St. Petersburg, Russia}
\affiliation{$^{42}$Stockholm University, Stockholm, Sweden, and
                Uppsala University, Uppsala, Sweden}
\affiliation{$^{43}$Lancaster University, Lancaster, United Kingdom}
\affiliation{$^{44}$Imperial College, London, United Kingdom}
\affiliation{$^{45}$University of Manchester, Manchester, United Kingdom}
\affiliation{$^{46}$University of Arizona, Tucson, Arizona 85721, USA}
\affiliation{$^{47}$California State University, Fresno, California 93740, USA}
\affiliation{$^{48}$University of California, Riverside, California 92521, USA}
\affiliation{$^{49}$Florida State University, Tallahassee, Florida 32306, USA}
\affiliation{$^{50}$Fermi National Accelerator Laboratory,
                Batavia, Illinois 60510, USA}
\affiliation{$^{51}$University of Illinois at Chicago,
                Chicago, Illinois 60607, USA}
\affiliation{$^{52}$Northern Illinois University, DeKalb, Illinois 60115, USA}
\affiliation{$^{53}$Northwestern University, Evanston, Illinois 60208, USA}
\affiliation{$^{54}$Indiana University, Bloomington, Indiana 47405, USA}
\affiliation{$^{55}$University of Notre Dame, Notre Dame, Indiana 46556, USA}
\affiliation{$^{56}$Purdue University Calumet, Hammond, Indiana 46323, USA}
\affiliation{$^{57}$Iowa State University, Ames, Iowa 50011, USA}
\affiliation{$^{58}$University of Kansas, Lawrence, Kansas 66045, USA}
\affiliation{$^{59}$Kansas State University, Manhattan, Kansas 66506, USA}
\affiliation{$^{60}$Louisiana Tech University, Ruston, Louisiana 71272, USA}
\affiliation{$^{61}$University of Maryland, College Park, Maryland 20742, USA}
\affiliation{$^{62}$Boston University, Boston, Massachusetts 02215, USA}
\affiliation{$^{63}$Northeastern University, Boston, Massachusetts 02115, USA}
\affiliation{$^{64}$University of Michigan, Ann Arbor, Michigan 48109, USA}
\affiliation{$^{65}$Michigan State University,
                East Lansing, Michigan 48824, USA}
\affiliation{$^{66}$University of Mississippi,
                University, Mississippi 38677, USA}
\affiliation{$^{67}$University of Nebraska, Lincoln, Nebraska 68588, USA}
\affiliation{$^{68}$Princeton University, Princeton, New Jersey 08544, USA}
\affiliation{$^{69}$State University of New York, Buffalo, New York 14260, USA}
\affiliation{$^{70}$Columbia University, New York, New York 10027, USA}
\affiliation{$^{71}$University of Rochester, Rochester, New York 14627, USA}
\affiliation{$^{72}$State University of New York,
                Stony Brook, New York 11794, USA}
\affiliation{$^{73}$Brookhaven National Laboratory, Upton, New York 11973, USA}
\affiliation{$^{74}$Langston University, Langston, Oklahoma 73050, USA}
\affiliation{$^{75}$University of Oklahoma, Norman, Oklahoma 73019, USA}
\affiliation{$^{76}$Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\affiliation{$^{77}$Brown University, Providence, Rhode Island 02912, USA}
\affiliation{$^{78}$University of Texas, Arlington, Texas 76019, USA}
\affiliation{$^{79}$Southern Methodist University, Dallas, Texas 75275, USA}
\affiliation{$^{80}$Rice University, Houston, Texas 77005, USA}
\affiliation{$^{81}$University of Virginia,
                Charlottesville, Virginia 22901, USA}
\affiliation{$^{82}$University of Washington, Seattle, Washington 98195, USA}


==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                         7/7/09
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
\bibitem[a]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA.
\bibitem[b]{askew,atramentov,gershtein}
Visitor from Rutgers University, Piscataway, NJ, USA.
\bibitem[c]{burdin}
Visitor from The University of Liverpool, Liverpool, UK.
\bibitem[d]{luna-garcia}
Visitor from Centro de Investigacion en Computacion - IPN,
  Mexico City, Mexico.
\bibitem[e]{podesta-lerma}
Visitor from ECFM, Universidad Autonoma de Sinaloa, Culiac\'an, Mexico.
\bibitem[f]{weber}
Visitor from Universit{\"a}t Bern, Bern, Switzerland.
\bibitem[g]{wenger}
Visitor from Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland.
%\bibitem[?]{coadou}
%Visitor from CERN, Geneva, Switzerland.
%\bibitem[?]{hooper}
%Visitor from Bradley University, Peoria, IL, USA.
%\bibitem[?]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA.
%\bibitem[\ddag]{deceased}
%Deceased.

%
\vskip 0.25cm

